Predicting Flat-Fading Channels via Meta-Learned Closed-Form Linear Filters and Equilibrium Propagation

Predicting fading channels is a classical problem with a vast array of applications, including as an enabler of artificial intelligence (AI)-based proactive resource allocation for cellular networks. Under the assumption that the fading channel follows a stationary complex Gaussian process, as for Rayleigh and Rician fading models, the optimal predictor is linear, and it can be directly computed from the Doppler spectrum via standard linear minimum mean squared error (LMMSE) estimation. However, in practice, the Doppler spectrum is unknown, and the predictor has only access to a limited time series of estimated channels. This paper proposes to leverage meta-learning in order to mitigate the requirements in terms of training data for channel fading prediction. Specifically, it first develops an offline low-complexity solution based on linear filtering via a meta-trained quadratic regularization. Then, an online method is proposed based on gradient descent and equilibrium propagation (EP). Numerical results demonstrate the advantages of the proposed approach, showing its capacity to approach the genie-aided LMMSE solution with a small number of training data points.

==> app_for_future.tex <==
\subsection{Closed-Form Solution}
The most straight forward way is to directly obtain $\bar{v}^*_{\lambda}$ in \eqref{eq:closed_from_sol_meta_scalar} with $\{\mathcal{Z}_{f'}\}_{f'=\min{(f-M,1)}}^{f-1}$ in lieu of $\{\mathcal{Z}_f\}_{f=1}^F$. Precisely, the update rule for hyperparameter vector $\bar{v}$ at frame $f$ can be expressed as
\begin{align}
    \bar{v}_{\lambda,M}^*(f) = \argmin_{\bar{v}} \sum_{f'=\max{(f-M,1)}}^{f-1} \norm{\tilde{X}_{f'}^\text{te}\bar{v} - \tilde{y}_{f'}^\text{te}}^2.
    \label{eq:online_closed_1}
\end{align}
However, as this cannot retain the information from the out-of-memory frames $f' < f-M$, alternative approaches need to be considered.

\subsection{Closed-Form Solution via Ridge Regression}
Here we modify \eqref{eq:online_closed_1} so that $\bar{v}_{\lambda}^*(f)$ can capture frames outside of the memory via regularization with the previous hyperparameter vector $\bar{v}^*_\lambda(f-1)$, i.e.,
\begin{align}
    \bar{v}^{*,\text{ridge}}_{\lambda,M}(f) &= \argmin_{\bar{v}} \sum_{f'=\max{(f-M,1)}}^{f-1} \left\{ \norm{\tilde{X}_f^\text{te}\bar{v} - \tilde{y}_f^\text{te}}^2 + \lambda' \norm{\bar{v}-\bar{v}^{*,\text{ridge}}_{\lambda,M}(f-1)}^2\right\},
\label{eq:online_closed_2}
\end{align}
with $\bar{v}^{*,\text{ridge}}_{\lambda,M}(1) = \bar{v}_{\lambda,M}^*(1)$ from \eqref{eq:online_closed_1}.

%%%%%%%%%%%


Via GD with $g_f^{\text{meta-EP}}$, the update rule for hyperparameter vector $\bar{v}$ at frame $f$ and iteration $k$, denoted as $\bar{v}_{\lambda,f,M}^{(k)}$, can be expressed as
\begin{align}
    \bar{v}_{\lambda,f,M}^{(k+1)} = \bar{v}_{\lambda,f,M}^{(k)} - \eta_{\lambda,f,M}^{(k)} \sum_{f'=\max{(f-M,1)}}^{f-1} g_{f'}^{\text{meta-EP}}\big(\bar{v}_{\lambda,f,M}^{(k)}\big),
    \label{eq:gd_implicit}
\end{align}
with step size $\eta_{\lambda,f,M}^{(k)} > 0$. After sufficient iterations with proper step size, $\bar{v}_{\lambda,f,M}^{(k)}$ converges to $\bar{v}_{\lambda,M}^*(f)$ as \eqref{eq:obj_for_gradient_methods} is the convex problem. Overall the EP-based meta-learning procedure is described in Algorithm~\ref{alg:scalar_meta_learning_GD} with $M=F$ and at $f=F+1$. To facilitate the online learning throughout the frames $f=1,2,\ldots$, we further consider the following online update rule
\begin{align}
    \bar{v}^{*,\text{EP}}_{\lambda,M}(f) = \bar{v}^{(K)}_{\lambda,f,M}, \text{ with } \bar{v}_{\lambda,f,M}^{(0)}=\bar{v}^{*,\text{EP}}_{\lambda,M}(f-1),
    \label{eq:online_ep_GD}
\end{align}
with per-frame iteration number $K>0$.

%%%%%%%%
\begin{algorithm}[h] %!
\DontPrintSemicolon
\smallskip
\KwIn{meta-training data  $\{\{ h_{l,f} \}_{l=1}^{L+N+\delta-1}\}_{f=1}^F$; training set size $L^\textrm{tr}$; test set size $L^\textrm{te} = L-L^\textrm{tr}$; window size $N$; prediction lag size $\delta$; hyperparameter $\lambda > 0$, $\alpha \neq 0$}
\KwOut{meta-learned bias vector $\bar{v}^{(k)}$}
\vspace{0.15cm}
\hrule
\vspace{0.25cm}
%fist phase
\textbf{initialize} $\bar{v}^{(0)}$, \textbf{split} $\mathcal{Z}_f$ into training set $\mathcal{Z}_f^\text{tr}$ and test set $\mathcal{Z}_f^\text{te}$ for all $f \in \{1,\ldots,F\}$ \\
$k=0$\\
\While{{\em convergence criterion not satisfied}}{
\For{{\em each frame $f \in \{1,\ldots,F\}$}}{
obtain weighted stacked input matrix $X_f^\alpha = [X_f^\text{tr}, \alpha X_f^\text{te}]^\top$ and weighted stacked target vector $y_f^\alpha = [y_f^\text{tr}, \alpha y_f^\text{te}]^\top$
\\
solve ridge regression problem \eqref{eq:general_ridge} with $X_f^\alpha$ and $y_f^\alpha$ in lieu of $X$ and $y$ to obtain $v_f^{\alpha,\bar{v}^{(k)}}$ \\
solve ridge regression problem \eqref{eq:general_ridge} with $X_f^\text{tr}$ and $y_f^\text{tr}$ in lieu of $X$ and $y$ to obtain $v_f^{0,\bar{v}^{(k)}}$ \\
compute $g_f^\text{meta-EP}(\bar{v}^{(k)}) = \frac{1}{\alpha} \left(2\lambda(v_f^{0,\bar{v}^{(k)}} - v_f^{\alpha,\bar{v}^{(k)}})\right)$
}
update bias vector
\begin{align}
    \nonumber
    \bar{v}^{(k+1)} = \bar{v}^{(k)} - \eta^{(k)} \sum_{f=1}^F g_f^{\text{meta-EP}}(\bar{v}^{(k)}),
\end{align}
$k \leftarrow k + 1$
}

\caption{Meta-learning for scalar channel prediction via gradient descent}
\label{alg:scalar_meta_learning_GD}
\end{algorithm}


==> noisy.tex <==
\section{Incorporating Estimation Noise}
\label{sec:noisy}
Until now, we have assumed that channel vectors $\{ h_{l,f} \}_{l=1}^{L+N+\delta-1}$ are available noiselessly to the predictor for each frame $f$. In practice, channel information needs to be estimated via pilots. To elaborate on this point, let us assume the received signal model
\begin{align}
    y_{l,f}[i] = h_{l,f} x_{l,f}[i] + n_{l,f}[i],
    \label{eq:channel_model_pilot}
\end{align}
where $x_{l,f}[i]$ stands for the $i$th transmitted pilot symbol in block $l$ of frame $f$; $y_{l,f}[i]$ for the corresponding received symbol; and we have additive white complex Gaussian noise $n_{l,f}[i] \sim \mathcal{CN}(0,N_0)$. Given an average energy constraint $\mathbb{E}[|x_{l,f}[i]|^2]=E_x$ for the training symbol, the average signal-to-noise ratio (SNR) is given as $E_x/N_0$. From \eqref{eq:channel_model_pilot}, we can estimate the channel via a maximum likelihood, or least squares, estimation as
\begin{align}
\check{h}_{l,f} = \frac{y_{l,f}[i]}{x_{l,f}[i]} = h_{l,f} + \frac{n_{l,f}[i]}{x_{l,f}[i]} = h_{l,f} + \xi,
\end{align}
which if affected by the channel estimation noise $\xi \sim \mathcal{CN}(0, \text{SNR}^{-1})$. If $P$ training symbols are available in each block, the channel estimation noise can be reduced via averaging to $\text{SNR}^{-1}/P$. The noisy channels $\tilde{h}_{l,f}$ can be used as training data in the algorithms described in the previous subsections.
